Analyzing Defense Strategies Against Mobile Information Leakages: A Game-Theoretic Approach

Abuse of zero-permission sensors on-board mobile and wearable devices to infer users' personal context and information is a well-known privacy threat that has received significant attention. Efforts towards protection mechanisms that prevent or limit the success of such threats, however, have been ad-hoc so far and have primarily focused on designing threat-specific customized defense mechanisms. Such approaches are not very practical, as evident from their limited adoption within major mobile/wearable operating systems. In the end, it is clear that all privacy threats that take advantage of unrestricted access to zero-permission sensors can be prevented if access to these sensors is regulated. However, due to the dynamic nature of sensor usage and requirements of different mobile applications, design of such access control mechanisms is not trivial. To effectively design an automated mobile defense mechanism that can dynamically measure the threat level of different sensor access requests from different applications and appropriately block suspicious requests, the problem of zero-permission sensor access needs to be first formally defined and analyzed. This paper accomplishes the above objective by employing game theory, specifically, signaling games, to analytically model the sensor access scenario for mobile applications, including, formalizing sensor access strategies of mobile applications and defense strategies of the on-board defense mechanism and the associated costs and benefits. Within the confines of a formal and practical game model, the paper then outlines conditions under which equilibria can be achieved between entities (applications and defense mechanism) with conflicting goals. The game model is further analyzed using numerical simulations, and also extended in the form of a repeated signaling game.

==> discussion.tex <==
\section{Practical Considerations}
The analytical and numerical results, outlined so far, sheds light on the strategic sensor access behavior of different applications, strategic access control response from the defense mechanism, and the resulting payoffs (benefits or losses) for the involved entities due to their actions. A critical practical challenge for the defense mechanism to act in a strategically optimal manner (as outlined in the various game solutions) is the accurate determination (or quantification) of the Nature's selection probability $\theta$.
%however lies in the  of a accurate  from 's perspective. 
As the defense mechanism is unable to infer the application type (malicious or honest) by itself, solely by looking at the incoming signal (or sensor access requests) and as there is no feedback on the applications' past conduct when given access, it has to determine $\theta$ from external contexts.
%does not know applications' true intentions when they request sensor data, and what they conduct with the sensor data if given access, . 
One technique the defense mechanism can use to estimate $\theta$ is to employ aggregated \textit{reputation} of all currently installed applications, obtained from external sources such as app stores \cite{pranata2012determining,frank2012mining}.

%The second practical consideration that needs to be highlighted here is that our current game model ($\mathbb{G}_D$) is a single stage (shot) game, however, in real-life implementations such a single shot game will be repeated every time some application requests sensor access. In most signaling game use-cases in the literature, the belief functions are updated based on the outcome of the game(s) played in earlier stages or rounds. However, in our use-case and current model, the defense mechanism has no provision of determining the outcome(s) of the previous games. In real-life scenarios, the defense mechanism may not be even aware if the user's personal information is leaked by an application, in real-time. Most leakages and inferences of private user data, as evident from the literature \cite{MarquardtVCT:2012,MiluzzoVBC:2012,wang2015,maiti:2016,MaitiJHB:2018,MaitiHSJ:2018}, are carried out in an offline and non real-time fashion, at a later point in time. Moreover, the adversary may (mis)use the stolen private information at a much later time. However, if the defense mechanism uses reputation-based $\theta$ calculations, it can dynamically update its calculations whenever a change in aggregated reputation (of applications) is detected, say from an external source such as an app store. For example, when a new application is installed, an existing application is uninstalled, or an installed application's reputation drops due to known malicious intent \cite{spyapps}.


%In future work, we can design a belief updating mechanism which will update the beliefs of the defender after each stage of the game and making the system to converge to an equilibrium stage. We can design the belief updating mechanism in such a way that it takes into account the type of request being made by the application, prior beliefs of the defender and the current action of the application to update the $\theta$ or the beliefs of the defender. The type of the requests made by an application can be asking for the normal navigation data, gyroscopic data, etc or an application can also make suspicious requests like asking users personal information, credit card information, etc. So, the designed belief updating mechanism can take these three as inputs and the resulting output can be feeded to the defender so that it can update the beliefs or updating mechanism can update the $\theta$ by itself, resulting in the automatic update of the beliefs.  
 
%It can only determine the type after it sees the request made by the application.  The PBNE  is defined by  player 1 action and the corresponding best response from the defender in different conditions. So, in real life a defender can come across a separating , pooling, hybrid or mixed (not discussed) strategy profiles and the above equilibrium results shows the decisions which a defender can take. As a result, those decisions can either lead to an equilibrium or not. 

%In this work, our main aim was to design a system which will help block the malicious applications requests and reach an equilibrium state.The above analytical and empirical results shows that our system was able to thwart malicious applications requests and also increasing the defenders expected utility and HA payoff as we increase the value of $\theta$. 


%$\theta$ value directly impacts the number of malicious applications and honest applications in a system. One can also define $\theta$ in terms of the number of requests a malicious application is making. Lets consider an example, a mobile phone having number of malicious applications more than the number of honest applications, thereby implying the value of $\theta$ will be greater than 0.5. Nature is basically a system which determines the value of $\theta$ , thus also determining the number of malicious applications or honest applications in the system. If we follow the defender we have designed and look at the graphs in Fig 3, we can see as the value of $\theta$ increases, the defender starts blocking the suspicious requests. Thereby increasing the expected utility of the defender, decreasing the MA payoff and increasing the payoff of HA. Our system is a single shot system, i.e. we don't update the beliefs after each stage of the game, but one can implement it in their own environment and can gradually reduce the $\theta$ so that requests from malicious applications will become less in number. There are lots of applications of Google Play store, some of them may be malicious. So, one can also deploy our designed defender in this particular environment for reducing the suspicious requests from malicious applications. However, there are certain limitations in the proposed design which we have discussed below.





%\section{Discussion}
%\label{sec:discussion}

%\subsection{Limitations}
%We have not analyzed mixed equilibrium in the proposed design. Mixed equilibrium is one in which both types of player 1 randomizes between the signal they send. In our case, both MA and HA randomizes between the suspicious and non-suspicious request. 
%We are also not updating the beliefs of the defender after each stage of the game i.e not using the belief updating mechanism. The reason is since the belief updating mechanism will be automated, so there will always be a mixed equilibrium and separating and pooling equilibrium will not apply to this specific scenario. This is also one of the reason why we are not analyzing the mixed strategy.
%The parametric values we chose was to show the patterns observable across the three equilibrium strategies. We don't know whether these parameter values will apply to real scenario as well.

%\subsection{Future Work}
%\label{sec:future_work}
%In future work, we can design a belief updating mechanism which will update the beliefs of the defender after each stage of the game and making the system to converge to an equilibrium stage. We can design the belief updating mechanism in such a way that it takes into account the type of request being made by the application, prior beliefs of the defender and the current action of the application to update the $\theta$ or the beliefs of the defender. The type of the requests made by an application can be asking for the normal navigation data, gyroscopic data, etc or an application can also make suspicious requests like asking users personal information, credit card information, etc. So, the designed belief updating mechanism can take these three as inputs and the resulting output can be feeded to the defender so that it can update the beliefs or updating mechanism can update the $\theta$ by itself, resulting in the automatic update of the beliefs.   

==> simulation.tex <==
% !TeX root = BC_PGG_July2018.tex
\section{Numerical Analysis}
\label{sec:Sim}

We conduct some simple numerical analysis, in order to show the performance of the proposed algorithm comparing to standard shard-based protocols. We assume that 1000 processors are actively participating in a shard-base public  permissionless  blockchain. We assume that these processors are distributed in 10 shards according to Elastico protocol. We also assume that each processor receives $x_i$ transactions which follow a Gaussian distribution with mean of $1000$ and $100$ standard deviation. Table~\ref{tab:values} shows other values for parameters in our numerical evaluations.  Figure~\ref{fig_sim1} shows the average payoff of cooperative and defective processors when they foloow uniform distribution of rewards. Our numerical results show that by employing incentivized protocol, processors can obtain highre payoff. 



\begin{table}[t]
\caption{Values of parameters in the numerical evaluations.}
\begin{center}
\begin{tabular}{c | c | c | c | c | c} \toprule
 $BR$  & $c^m$ & $c^f$ & $c^v$ & $r$ & $N$   \\  \rowcolor[gray]{.9} \hline
$10000$         & $10$ & $10$ & $0.001$ & $0.1$ & $1000$
\end{tabular}
\end{center}
\label{tab:values}
\end{table}




\begin{figure}[t]
	\centering
	\includegraphics[scale=0.5]{Figures/freeloading.pdf}
	\caption{}
	\label{fig_sim1}
\end{figure}

%
%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.5]{Figures/nomorefreeloading.pdf}
%	\caption{}
%	\label{fig_sim1}
%\end{figure}
